Stable Code Technical Report

We introduce Stable Code, the first in our new-generation of code language models series, which serves as a general-purpose base code language model targeting code completion, reasoning, math, and other software engineering-based tasks. Additionally, we introduce an instruction variant named Stable Code Instruct that allows conversing with the model in a natural chat interface for performing question-answering and instruction-based tasks. In this technical report, we detail the data and training procedure leading to both models. Their weights are available via Hugging Face for anyone to download and use at https://huggingface.co/stabilityai/stable-code-3b and https://huggingface.co/stabilityai/stable-code-instruct-3b. This report contains thorough evaluations of the models, including multilingual programming benchmarks, and the MT benchmark focusing on multi-turn dialogues. At the time of its release, Stable Code is the state-of-the-art open model under 3B parameters and even performs comparably to larger models of sizes 7 billion and 15 billion parameters on the popular Multi-PL benchmark. Stable Code Instruct also exhibits state-of-the-art performance on the MT-Bench coding tasks and on Multi-PL completion compared to other instruction tuned models. Given its appealing small size, we also provide throughput measurements on a number of edge devices. In addition, we open source several quantized checkpoints and provide their performance metrics compared to the original model.

==> tabs/tab_arch_train_config.tex <==
\begin{table}
\centering
\noindent
\begin{tabular}{P P P P G}\toprule
\textbf{Parameters} & \textbf{Hidden Size} & \textbf{Layers} & \textbf{Heads} & \textbf{Sequence Length} \\[0.1ex]
\midrule
1,644,417,024 & 2048 & 24 & 32 & 4096 \\ [1ex]
\midrule
\end{tabular}
\caption{Stable LM 2 model architecture.}
\label{tab:architecture-layout}
\begin{tabular}{H H H H}
\toprule
\textbf{Data Parallel Degree} & \textbf{Micro Batch Size} & \textbf{Gradient Accumulation Steps} & \textbf{Activation Checkpointing} \\[0.1ex]
\midrule
512 & 2 & 2 & disabled \\ [0.1ex]
\midrule
\end{tabular}
\caption{Stable LM 2 training configuration.}
\label{tab:training-config}
\end{table}

==> tabs/tab_llama_multipl.tex <==
\begin{xltabular}{\textwidth}{l|r|c| *{6}{c} r}
\caption{Performance Comparison of Stable Code and Code Llama on Multi-PL} \label{tab:performance-largebase} \\
\toprule
Model & Size & Avg & \rotatebox{0}{Python} & \rotatebox{0}{C++} & \rotatebox{0}{JavaScript} & \rotatebox{0}{Java} & \rotatebox{0}{PHP} & \rotatebox{0}{Rust} \\
\midrule
\endfirsthead
\toprule
\endhead
% \bottomrule
% \multicolumn{10}{r}{{Continued on next page}} \\
% \endfoot
% \bottomrule
% \endlastfoot
% \midrule
Stable Code & 3B & 29.1& 32.4\% &  30.9\% & 32.1\% &\textbf{ 32.1\%} & 24.2\% & 23.0\% \\
Code Llama & 7B & 29.1& 30.0\% & 28.2\% & \textbf{32.5\%} & 31.9\% & 25.7\% & \textbf{26.3\%}\\
Star Coder & 15B & 29.0& \textbf{33.6} \% & \textbf{31.6\%} & 30.8\% & 30.2\% & \textbf{26.1\%} & 21.8\%\\
\midrule

\end{xltabular}

==> tabs/tab_long_ctx_data.tex <==
\begin{table}[ht]
\centering
\noindent
\begin{tabular}{G N G N N N}
\toprule
%\begin{tabular}{N N N N N }\toprule
\multicolumn{1}{ c }{\textbf{Dataset}} & \textbf{Sampling Weight} & \textbf{Num Tokens Sampled} & \textbf{Epochs} & \textbf{Category}\\[1ex] 
\cmidrule(lr){1-1}
\cmidrule(lr){2-5}
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder C}} & 0.0924 & 122,202,657,912.00 &6.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder CPP}} & 0.0734 & 97,032,316,152.00 &6.0& Code\\ [0.2ex] 
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Java}} & 0.1029 & 136,010,698,326.00 &6.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Javascript}} & 0.0858 & 113,469,977,934.00 &6.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder CSS}} & 0.0146 & 19,285,266,328.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Go}} & 0.0258 & 34,092,166,492.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder HTML}} & 0.0298 & 39,354,336,188.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Ruby}} & 0.0061 & 8,011,730,332.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Rust}} & 0.0122 & 16,131,445,656.00 &6.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Markdown}} & 0.1154 & 152,629,435,716.00 &6.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Shell}} & 0.0033 & 4,323,112,416.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Php}} & 0.0764 & 100,958,420,706.00 &6.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Sql}} & 0.0247 & 32,645,285,202.00 &6.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder R}} & 0.0003 & 415,957,896.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Typescript}} & 0.0224 & 29,634,722,636.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Python}} & 0.1067 & 141,067,150,184.00 &8.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Jupyter}} & 0.0060 & 7,941,540,044.00 &4.0& Code\\ [0.2ex]
\rowcolor{Yellow}
\multicolumn{1}{ l }{\textbf{StarCoder Restructured Text}} & 0.0032 & 4,179,202,492.00 &4.0& Code\\ [0.2ex]
\cmidrule(lr){1-1}
\cmidrule(lr){2-5}

\rowcolor{Purple}
\multicolumn{1}{ l }{\textbf{Github Issues}} &0.0231&46,302,993,820 &2.5& Technical\\ [0.2ex]
\rowcolor{Purple}
\multicolumn{1}{ l }{\textbf{Github Diffs}} &0.0019&3,817,060,582 &2.0& Technical\\ [0.2ex] 
\rowcolor{Purple}
\multicolumn{1}{ l }{\textbf{StackExchange}} &0.0019&3,817,060,582 &2.0& Technical\\ [0.2ex] 
\cmidrule(lr){1-1}
\cmidrule(lr){2-5}
\rowcolor{LightCyan}
\multicolumn{1}{ l }{\textbf{Proof Pile}} & 0.0384 & 50,780,637,096 &1.0& Math\\ [0.2ex] 
\rowcolor{LightCyan}
\multicolumn{1}{ l }{\textbf{Meta Math QA}} & 0.0003 & 83,663,501 &4.0& Math\\ [0.2ex] 
\cmidrule(lr){1-1}
\cmidrule(lr){2-5}
\rowcolor{Pink}
\multicolumn{1}{ l }{\textbf{Arxiv}} & 0.0213 & 28,097,511,912.00 &1.0& Web\\ [0.2ex] 
\rowcolor{Pink}
\multicolumn{1}{ l }{\textbf{Refined Web}} & 0.0220 & 29,114,185,066.13 &0.5& Web\\ [0.2ex] 
\cmidrule(lr){1-1}
\cmidrule(lr){2-5}
\rowcolor{Brown}
\multicolumn{1}{ l }{\textbf{Instruction}} & 0.0006 & 819,864,748.00 &3.0& Instruction\\ [0.2ex] 
\midrule
\multicolumn{1}{ l }{\textbf{Total}} & 1 &1,322,090,182,830.13 && -\\ [0.2ex] 
\end{tabular}
\caption{The complete Stable LM 2 training set with sampling weights. The tokens count refers to the \textbf{NeoX} tokenizer introduced in Sec.~\ref{sec:tokenizer}}
\label{tab:data-mix}
\end{table}

==> tabs/tab_safe_eval.tex <==
\begin{xltabular}{\textwidth}{l|r| *{1}{c} r}
\caption{Evaluation of popular models and Stable Code Instruct 3B on Safe-Eval} \label{tab:safe-eval-transposed} \\
\toprule
Model & Score \\
\midrule
\endfirsthead
\toprule
\endhead

\bottomrule
\multicolumn{8}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot

Stable Code Instruct 3B & 28.0\% \\
DeepSeek-Coder Instruct 1.3B & 24.0\% \\
SQLCoder 7B & 64.0\% \\
\end{xltabular}

